Employing polyhedral methods to optimize stencils on FPGAs with stencil-specific caches, data reuse, and wide data bursts

It is well known that to accelerate stencil codes on CPUs or GPUs and to exploit hardware caches and their lines optimizers must find spatial and temporal locality of array accesses to harvest data-reuse opportunities. On FPGAs there is the burden that there are no built-in caches (or only pre-built hardware descriptions for cache blocks that are inefficient for stencil codes). But this paper demonstrates that this lack is also a chance as polyhedral methods can be used to generate stencil-specific cache-structures of the right sizes on the FPGA and to fill and flush them efficiently with wide bursts during stencil execution. The paper shows how to derive the appropriate directives and code restructurings from stencil codes so that the FPGA compiler generates fast stencil hardware. Switching on our optimization improves the runtime of a set of 10 stencils by between 43x and 156x.

==> Makefile <==
PAPER_TEX = main.tex
PAPER_PDF = main.pdf

TRASH_FILES = *.blg *.fls *.aux *.log *.nav *.out *.snm *.toc *.lst *.vrb *.off *fdb_latexmk
PDFLATEX_OPTIONS = -halt-on-error -file-line-error

# let latexmk do the dependency detection
.PHONY: all

all: paper talk

.PHONY: paper
paper: mktemp
	latexmk -pdf -pdflatex="pdflatex $(PDFLATEX_OPTIONS)" $(PAPER_TEX)

.PHONY: bw
bw: all
	gs -sOutputFile=main_bw.pdf \
		-sDEVICE=pdfwrite -sColorConversionStrategy=Gray \
		-dProcessColorModel=/DeviceGray -dCompatibilityLevel=1.4 \
		-dNOPAUSE -dBATCH $(PAPER_PDF)

.PHONY: preview
preview: mktemp
	latexmk -pvc -pdf -pdflatex="pdflatex $(PDFLATEX_OPTIONS)" $(PAPER_TEX)

.PHONY: spellcheck
spellcheck:
	for i in **/*.tex *.tex; do  \
		cat "$$i" | aspell -a --lang=EN check > $$i_spell_report.txt; \
	done

.PHONY: mktemp
mktemp:
	mkdir -p _tmp

.PHONY: distclean
distclean: clean
	rm -f $(PAPER_PDF)

PACK_FILES = tables references config content text llncs.cls main.tex Makefile splncs04.bst main.pdf talk/talk.pdf
.PHONY: pack
pack: paper talk
	tar -c -f "mayer_brandner_hellmann_schwarzer_philippsen.tar" $(PACK_FILES)

.PHONY: clean
clean:
	rm -f $(TRASH_FILES)
	rm -rf _tmp


.PHONY: talk
talk:

.PHONY: add
add:
	git add main.tex content/*.tex Makefile


==> wrapfigure.tex <==
\setlength{\intextsep}{1ex}
